Integrative Few-Shot Learning for Classification and Segmentation

We introduce the integrative task of few-shot classification and segmentation (FS-CS) that aims to both classify and segment target objects in a query image when the target classes are given with a few examples. This task combines two conventional few-shot learning problems, few-shot classification and segmentation. FS-CS generalizes them to more realistic episodes with arbitrary image pairs, where each target class may or may not be present in the query. To address the task, we propose the integrative few-shot learning (iFSL) framework for FS-CS, which trains a learner to construct class-wise foreground maps for multi-label classification and pixel-wise segmentation. We also develop an effective iFSL model, attentive squeeze network (ASNet), that leverages deep semantic correlation and global self-attention to produce reliable foreground maps. In experiments, the proposed method shows promising performance on the FS-CS task and also achieves the state of the art on standard few-shot segmentation benchmarks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sec/99_cabinet.tex <==
% Each correlation tensor in the hypercorrelation pyramid $\{\bC^{(p)}\}_{p=1}^{P}$ is fed to a series of \ourlayer layers, and each of their correlational features are integrated into a single segmentation mask by cascaded upsampling and addition operations as similarly as \cite{fpn, hsnet, refinenet}, which reflects diverse contexts from multiple layers.
% \dahyun{The following paragraph is under revision}
\smallbreakparagraph{Attentive squeeze layer (\ourlayer layer).}
% We introduce our primitive building layer of our model, dubbed Query-Sliding Self-Attention layer (\ourlayer layer).
An \ourlayer layer takes a 2D spatial correlation pattern on the support dimension for each query dimension of an input correlation and transforms the 2D correlation pattern into another level of correlational representation of a smaller support dimension.
To give a model a holistic and structured view of the support feature correspondence with each query position, 
% To globally analyze the correlational features, 
we adopt the global self-attention mechanism~\cite{transformers} for correlational feature transform, \ie, the \ourlayer layer applies self-attention on the dense feature correlation domain.

Given a correlation tensor $\bC \in \Real^{C_{\text{in}} \times H_\textq \times W_\textq \times H_\texts \times W_\texts}$ in a hypercorrelation pyramid $\{\bC^{(p)}\}_{p=1}^{P}$, we start by embedding a correlation input to a target\footnote{
In this section, we adapt the term ``target'' to indicate the ``query'' embedding in the context of self-attention learning~\cite{transformers, vit, lsa, pvt} to avoid homonymous confusion with the ``query'' image to be segmented.
}
, key, value triplet: 
\begin{equation}    
% $
\bT, \bK, \bV \in \Real^{C_{\text{hd}} \times H_\textq \times W_\textq \times H_\texts' \times W_\texts'},
% $
\end{equation}
using three $1 \times 1 \times k \times k$ convolutions.
The convolutional embedding with a stride bigger than one governs the size reduction of the support dimension such that $H_\texts' \leq H_\texts$ and $W_\texts' \leq W_\texts$ while it \textit{slides} over the query dimension to broadcast the operation for all query positions.
Hence, the resolution of query dimension is preserved.
% As our goal is to transform the 2D support correlation into a point feature to embed in the query feature canvas, the resolution of query dimension is always preserved.
The resultant target and key correlational representations, $\bT$ and $\bK$, are then used to compute an attention context, and the attention context aggregates the value representation, $\bV$, to produce the next level of correlational representation.
An attention context map is designed to reflect relatedness within a correlation pattern size of  $H_\texts' \times W_\texts'$ on each query position, and thus the key range of the attention context is limited to the support feature dimensions only.
On the implementation side, the attention context is computed by matrix multiplication\footnote{\eqref{eq:sixd_attn} equals to $\bA = \mathrm{einsum}(\bT, \bK, \mathtt{chwij, chwkl \rightarrow hwij11kl}).$} between the last two dimensions of each $\bT$ and $\bK$ for each query position indices such that:
\begin{equation}
\bA = \bT \bK^{\top} \in \Real^{\overbrace{\scriptstyle{(H_\textq \times W_\textq \times H_\texts' \times W_\texts')}}^{\text{target range}} \times \overbrace{\scriptstyle{(1 \times 1 \times H_\texts' \times W_\texts')}}^{\text{key range}}},
\label{eq:sixd_attn}
\end{equation}
% which is equivalent to:
% \begin{equation}
% \bA = \mathrm{einsum}(\bT, \bK, \mathtt{chwij, chwkl \rightarrow hwij11kl}).
% \label{eq:sixd_attn_einsum}
% \end{equation}
To encourage the attention context to attend more on the foreground region among support positions, we leverage a strong mask prior if a support mask annotation $\bY_\texts$ is available.
The attention context $\bA$ is first reshaped to eliminate the dummy dimensions, masked by the support mask, and then normalized such that each key range sums to one:  
\begin{equation}
\bar{\bA}(\bp_\textq, \bp_\texts, \bu_\texts) = \frac{\exp \left( \bA(\bp_\textq, \bp_\texts, \bu_\texts) \bY(\bu_\texts) \right)}{\sum_{\bu_\texts'}\exp \left( \bA(\bp_\textq, \bp_\texts, \bu'_\texts) \bY(\bu'_\texts) \right)},
\label{eq:masked_attn}
\end{equation}
\begin{equation}
\text{where\, } \bY_\texts(\bu_\texts) =
\begin{cases}
  1 \quad \quad \; \text{if} \; \bu_\texts \in \Real^{H'_\texts \times W'_\texts} \text{ is foreground} \\    
  - \infty  \quad \text{otherwise.}
\end{cases}
\end{equation}
The masked-attention context $\bar{\bA}$ is then used to aggregate\footnote{\text{\eqref{eq:agg}} equals to $\bC_\textA = \mathrm{einsum}(\bar{\bA}, \bV, \mathtt{hwijkl, chwkl \rightarrow chwij})$} the value tensor $\bV$:
\begin{equation}
\bC_{\textA} = \bar{\bA} \bV \in \Real^{C_{\text{hd}} \times H_\textq \times W_\textq \times H_\texts' \times W_\texts'}.
\label{eq:agg}
\end{equation}
% which is equivalent to:
% \begin{equation}
% \bC_\textA = \mathrm{einsum}(\bar{\bA}, \bV, \mathtt{hwijkl, chwkl \rightarrow chwij}).
% \label{eq:agg_einsum}
% \end{equation}
The attended representation is fed to an MLP and added to the input, which is optionally being fed to a convolutional layer $\bW_\textI$ if either the channel or the spatial dimensions mismatches with that of output, followed by an activation layer $\varphi(\cdot)$ consisting of a normalization~\cite{groupnorm} and a non-linear activation~\cite{relu}:
\begin{equation}
\bC_\texto = \varphi(\bW_\texto(\bC_\textA) + \bW_\textI(\bC) ) \in \Real^{C_{\text{out}} \times H_\textq \times W_\textq \times H_\texts' \times W_\texts'}.
\end{equation}
The output then is fed to another feed-forwarding MLP that concludes a unit operation of a \ourlayer layer:
\begin{equation}
\bC' = \varphi(\bW_\text{FF}(\bC_\texto) + \bC_\texto) \in \Real^{C_{\text{out}} \times H_\textq \times W_\textq \times H_\texts' \times W_\texts'}.
\end{equation}
\ourlayer layers can be iteratively stacked to progressively reduce the correlation size of $H_\texts' \times W_\texts'$ on each query position to a smaller size.


\smallbreakparagraph{Multi-layer fusion.}
The pyramid correlational representations are merged from the coarsest to the finest level by cascading a pair-wise operation of the following three steps: upsampling, addition, and non-linear transform.
We first bi-linearly upsample the bottommost correlational representation to the query spatial dimension of its adjacent earlier one and then add the two representations to obtain a mixed one $\bC^{\text{mix}}$.
The mixed representation is fed to two parallel neural modules of which outputs are combined again by element-wise addition.
One branch is the proposed \ourlayer layer, and the other is a 2D convolution layer $\bW_\textq$, which produces a 2D output feature map of the same sizes of the input, for feature integration purpose within the mixed representation:
\begin{equation}
    \bC' = \mathrm{\ourlayer}(\bC^{\text{mix}}) + \bW_\textq(\mu(\bC^{\text{mix}})) \in \Real^{H_\textq \times W_\textq \times H_\texts' \times W_\texts' \times C},
    \label{eq:multi_layer_fusion}
\end{equation}
where $\mu$ denotes average-pooling over the support dimensions.
Note that the output of the convolution is broadcast along the support dimensions during element-wise addition.
This fusion layer is stacked twice until the support correlation map becomes an abstracted point feature, which is fed to the subsequent pyramidal fusion.
The output from the earliest fusion layer is fed to a convolutional decoder, which consists of interleaved 2D convolution and bi-linear upsampling that map the $C$-dimensional channel to 2 and the output spatial size to the input query size.
